On Social Optima of Non-Cooperative Mean Field Games

This paper studies the connections between mean-field games and the social welfare optimization problems. We consider a mean field game in functional spaces with a large population of agents, each of which seeks to minimize an individual cost function. The cost functions of different agents are coupled through a mean field term that depends on the mean of the population states. We show that under some mild conditions any $\epsilon$-Nash equilibrium of the mean field game coincides with the optimal solution to a convex social welfare optimization problem. The results are proved based on a general formulation in the functional spaces and can be applied to a variety of mean field games studied in the literature. Our result also implies that the computation of the mean field equilibrium can be cast as a convex optimization problem, which can be efficiently solved by a decentralized primal dual algorithm. Numerical simulations are presented to demonstrate the effectiveness of the proposed approach.

==> Meanfield.tex <==
\section{Social Optima in Mean Field Control}
This section employs the proposed reverse Stackelberg game to analyze the social optima in mean field control \cite{rammatico2016decentralized}.

Consider a mean field control problem \cite{rammatico2016decentralized}, where a large population of agents are coupled through an aggregative term. Each individual agent in this game has the following optimization problem:
\begin{align}
\label{eq:individualoptexmp}
&\max_{u_i} \sum_{k=1}^{K} \left(V_i^k(x_i(t_k))-\left(\dfrac{\sum_i^N u_i^k}{N}\right)^Tu_i^k \right)  \\
&\text{ subject to: } \nonumber\\
&\begin{cases}
{x}_{i}(t_{k})=A_i^kx_i(t_{k-1})+B_i^ku_i^k+C_i^k \\
0\leq u_i^k\leq \bar{u}_i,  \quad \forall k\in \mathcal{K}
\end{cases}
\end{align}
where the constraints $\mathcal{X}_i$ and $\mathcal{U}_i$ are convex sets. The mean field game (\ref{eq:individualoptexmp}) does not explicitly involve incentive strategy or leader objectives. However, comparing (\ref{eq:individualoptexmp}) and (\ref{eq:individualoptimization}), it is clear that the mean field game (\ref{eq:individualoptexmp}) can be regarded as a game with a special form of incentive strategy:
\begin{equation}
\label{meanfield}
\rho_k(\sum_{i=1}^N u_i)=\dfrac{1}{N} \sum_{i=1}^N u_i^k.
\end{equation}
Therefore, if we can construct a leader objective so that the corresponding reverse Stackelberg game (\ref{eq:socialwelfaremax}) has a solution that equals  the mean field control (\ref{meanfield}), then the mean field control is optimal over all other incentives strategies as it maximizes the social welfare.

Based on Theorem \ref{theorem2}, the solution of the reverse Stackelberg game satisfies $\rho(\cdot)=\mathcal{C}^{-1}(\cdot)$. Therefore, in order for $\rho(\cdot)$ to satisfy (\ref{meanfield}), we need $\mathcal{C}(p)=Np$. According to  the definition of $\mathcal{C}(\cdot)$ in (\ref{eq:coordinator_cp}), if we want $\mathcal{C}(p)=Np$, then the social cost function should be defined as follows:
\begin{equation}
\label{procurementcost}
\phi_k(z^k)=\dfrac{(z^k)^Tz^k}{2N},
\end{equation}
and the total resource constraint (\ref{eq:coordinator_cp2}) should be inactive (in other words, we can assume $D$ to be sufficiently large). Therefore, if the social cost function is defined as (\ref{procurementcost}), then we construct the following reverse Stackelberg game:
\begin{equation}
\label{eq:socialwelfaremax_exm}
\max_{\rho(\cdot)} \sum_{k=1}^{K} \sum_{i=1}^{N}V_{i}^k(x_i(t_k))-\sum_{k=1}^{K} \dfrac{(z^k)^Tz^k}{2N}
\end{equation}
\quad \quad \quad \quad \quad subject to: 
\begin{subnumcases}{}
\label{constraint10}
z^k=\sum\nolimits_{i=1}^N u_i^k \\
{x}_{i}(t_{k})=A_i^kx_i(t_{k-1})+B_i^ku_i^k+C_i^k \\
0\leq u_i^k\leq \bar{u}_i, \quad \forall i\in \mathcal{N}, \quad \forall k\in \mathcal{K}\\
u_i=u_i^*(\rho(\cdot)), \quad \forall i\in \mathcal{N},
\end{subnumcases}
and the mean field control scheme maximizes the social welfare (\ref{eq:socialwelfaremax_exm}). This can be summarized as follows:
\begin{theorem}
If the social cost function $\phi(\cdot)$ is defined as (\ref{procurementcost}), then the mean field control (\ref{meanfield}) induces an $\epsilon$-Nash equilibrium that maximizes the social welfare defined in (\ref{eq:socialwelfaremax_exm}).
\end{theorem}



\begin{remark}
The incentive strategy (\ref{meanfield}) in this section is the average of the agent {\bf control} decisions, but the mean field control typically characterizes the ``mass" behavior in terms of the average {\bf state} of the agents (followers). We clarify that proposed framework accommodates both cases. If we define the individual utility (\ref{eq:individualoptexmp}) as $J_i(u_i,u_{-i})=\sum_{k=1}^{K} \left( V_{i}^k(x_{i}(t_k))-\rho_k(\sum_{i=1}^N x_i(t_k))^Tx_i(t_k) \right)$, and the constraint  (\ref{constraint10}) to be  $z^k=\sum_{i=1}^N x_i(t_k)$, then it is easy to show that under the social cost function (\ref{procurementcost}), the mean field control scheme $\rho_k(\sum_{i=1}^N u_i)=\dfrac{1}{N} \sum_{i=1}^N x_i(t_k)$ induces an $\epsilon$-Nash equilibrium that maximizes the social welfare. 
In addition, although the proposed reverse Stackelberg game is deterministic and in discrete times, it can be generalized to continuous time and stochastic models. In this case, the state/control of the follower is a random variable, and the constraint (\ref{constraint10}) becomes the sum of the expectations of the individual state/control, which can be used to evaluate the social optima of mean field control in a stochastic setting \cite{huang2007large}. The details regarding this extension are left for future work. 
\end{remark}

